Multi-Emission Kernels for Parton Branching Algorithms

We introduce a general framework to construct multi-emission kernels for parton branching algorithms at the amplitude level and across different soft and collinear limits. We highlight the connection of kinematic parameterizations and recoil schemes to the underlying power counting, and discuss in detail how soft radiation can be partitioned in between different collinear configurations beyond the single-emission picture underpinning the traditional dipole and angular ordering approaches. Our work is a vital cornerstone to build parton branching algorithms which include multiply-unresolved emissions in a fully differential way, and our construction can also be used to obtain splitting functions for probabilistic algorithms or other cross-section level objects such as subtraction terms.

==> Makefile <==
all:
	pdflatex --shell-escape multi-emissions
	bibtex multi-emissions
	pdflatex --shell-escape multi-emissions

pdf:
	pdflatex --shell-escape multi-emissions
	bibtex multi-emissions
	pdflatex --shell-escape multi-emissions
	evince multi-emissions.pdf

ps:
	latex --shell-escape multi-emissions
	bibtex multi-emissions
	latex --shell-escape multi-emissions
	dvips multi-emissions

pdf-graphics:
	cd graphics
	for file in *.ps ; do pstopdf $$file ; done
	for file in *.eps ; do epstopdf $$file ; done
	cd ..

clean:
	rm -rf *~ *.aux *.log *.toc *.pdf *.dvi *.ps graphics/*.pdf

clean-bibtex:
	rm -rf *~ *.aux *.log *.toc *.bbl *.blg *.pdf *.dvi *.ps graphics/*.pdf

submit:
	if [ ! -e multi-emissions ]; then mkdir multi-emissions ; fi
	for file in *.tex *.bbl *.bib *.bst *.cls *.clo ; do \
	  cp $$file multi-emissions/ ; \
	done


